Investigating Inter-Satellite Link Spanning Patterns on Networking Performance in Mega-constellations

Low Earth orbit (LEO) mega-constellations rely on inter-satellite links (ISLs) to provide global connectivity. We note that in addition to the general constellation parameters, the ISL spanning patterns are also greatly influence the final network structure and thus the network performance. In this work, we formulate the ISL spanning patterns, apply different patterns to mega-constellation and generate multiple structures. Then, we delve into the performance estimation of these networks, specifically evaluating network capacity, throughput, latency, and routing path stretch. The experimental findings provide insights into the optimal network structure under diverse conditions, showcasing superior performance when compared to alternative network configurations.

==> data/results.tex <==
\section{Structure Analysis}


In this section, we evaluate the SNs performance affected by network structure in terms of coverage, collision risk, system throughput, and end-to-end latency.

We first analyze the coverage of networks with different structure.
Then we give the minimum distance between to encounter satellites which stands for the risk of collision.
Furthermore, the system throughput are given by calculating the capacity of each ISL.
We finally show the end-to-end latency in random connection pairs distributed in two satellites, and the path stretch is also provided to illustrate the detour of routing paths.
Our experiments were conducted using SNK\cite{snk}, a high-fidelity simulation and emulation framework that enables satellite networking emulation.


%本章，首先分析了不同结构网络的覆盖性
%然后，对eISL,sISL链路的长度以及容量进行了分析，特别针对eISL，还
%其次，针对不同尺度，不同相位因子，不同链路模式的星座，我们测量了其连通性
% 
% 

\subsection{Coverage Analysis}

\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=1.0\linewidth]{fig/coverage.png}
    \end{center}
    \caption{Coverage of constellation in different parameters.} 
        \label{fig:coverage}
 \end{figure}



                    % === coverage 的分析===

% --- 图1 a---
% 覆盖性中首先要分析的就是平均覆盖重数，即不同纬度地面站平均能接收到几个卫星的信号。
% 图1 所示为10，20,30,40密度下覆盖重数的变化，以及在20密度下不同相位因子下覆盖重数的变化。
%可以看到， density越高,平均覆盖数越大,且在倾角纬度上达到最高,如图1 a所示.
% 但相位因子并不影响平均覆盖重数，这也符合预计，因为卫星??

% --- 图1 b，c---
% 图1 b 所示，是密度为40^2在不同相位因子下，各个纬度地面站接收到卫星数量的方差。图1C为方差的平均值。可以看到，随着F从0到Fm的逐渐增高，方差也在逐渐增大，即每个地面站接收到卫星的卫星数量的变化逐渐增大，这也会给通信状态带来不稳定的情况，反映到网络层可能会使得jitter变大，从而导致数据报的重排序，从而明显影响通信质量。
% 因此，就此而言，相位因子应该尽量小，让地面站连接卫星数量保持在稳定数量。


% --- 纬度、F、尺度综合影响，待观察???---










\subsection{sISL Analysis}


\begin{figure}[htbp]

    \begin{center}
        
    \subfigure[sISL scale.]
    {
    \begin{minipage}{0.33\linewidth}
    \includegraphics[scale=0.2]{fig/range.png}%以这幅图的0.5倍大小输出
    \end{minipage}
    }\subfigure[sISL capacity.]
    {
    \begin{minipage}{.33\linewidth}
    \includegraphics[scale=0.2]{fig/capacity.png}%以这幅图的0.5倍大小输出
    \end{minipage}
    }\subfigure[Doppler Shift.]
    {
    \begin{minipage}{.33\linewidth}
    \includegraphics[scale=0.2]{fig/doppler.png}%以这幅图的0.5倍大小输出
    \end{minipage}
    } 


\end{center}

   

    \caption{Statistics of eISL between two encountering satellites.} 
       \label{fig:eISL_an}
   \end{figure}

   


% 我们还对不同结构的星座的链路进行了分析。

%           =======   ISL  =======
% 
% ---------------2.1. length and capacity-----------

% 图中所示为星间链路的长度统计，由于iISL长度比较统一，这里仅讨论sISL的长度。

% 图 2 a所示为sISL的长度统计，
% solid line是b=1链路;dash line 是b =0链路，dotted: b=m1; loosely dotted: b=m2黑色虚线则对应的iISL的长度分布以及链路容量统计.

% 可以看到，随着相位因子逐渐变大，b=1,b=0,b=m2链路（solid line）分布不变，而 b=m1 则逐渐变得不均匀
% 另外，随着相位因子增大，b=1,b=0链路尺度均值逐渐变大，而b=m1,b=m2则逐渐变小;
% 整体链路尺度大小为 bm1 < b0 < bm2 < b1

% 2 b为链路容量统计。
% 可以看到，随着相位因子逐渐变大，b=1,b=0,b=m2链路容量（solid line）分布不变，而 b=m1 则逐渐变得不均匀,这也导致其链路容量变化较大，可能会对网络带来较大的波动。
% 另外，随着相位因子增大，b=1,b=0链路容量均值逐渐变大，而b=m1,b=m2则逐渐变小;
% 整体链路容量大小为 bm1 > b0 > bm2>  b1


% ---------------2.2 速度 以及 多普勒频移-----------

% 图3 所示为链路中速度分布以及相应的多普勒频移，
% 
% 随遇链路的相位因子逐渐增大，b=1，b=0链路多普勒频移逐渐降低，而b=m1链路则逐渐变大，bm2逐渐变大，
% 且平均频移大小为 b=1 < b=0< b=m2 < b=m1
%
%
%----------3. 总结-------
% 综上，b0,bm1两条链路的容量，要远远大于b1和bm2，但bm1相对于b0，容量的稳定性稍差；
% 相应的，b1和bm2两条链路，频移更低，频率跟踪环的要求并不高，但容量较差，
% 在网络结构设计中，需要根据需求，权衡的选择。



% -- 转折
% 虽然已经分析了链路上的差异，但链路能极大的影响网络上的特征，从而全局的影响，我们对其进行探究。



\subsection{Network performance evaluation}

% 这里对连通性包括两个，连通均匀性，与连通充分性
%充分性，是通过增加网络内链路数量实现；
% 而均匀性，则是通过更好的设计星间互联实现

%                        ========   conn  ================

%                         -----3.1 四种链路的方向性分析-------

% 针对链路中不同，本节主要分析链路的方向性问题。

%图中所示为链路方向的概率密度图
% 图a是F=0的，图B是F=Fm的。
% 可以看到，iISL链路在倾角方向（i=53d）提供了最大比例的链路
% F=0时，链路方向分布范围较大，且b0链路全部处于水平，这为东西方向提供了足够好的连通性。
% F=Fm时，链路方向分布逐渐趋近于一致，这会导致网络的均匀性变差

%                  --------- 3.2 两两组合后的连通方向性 R---------
% 为了获得更高的吞吐量，采用*Grid 的ISL pattern更为实际，这就需要将上述sISL两两组合了。
% 为了探究在*Grid模式下，最好的ISL pattern， 我们好奇其均匀性表现如何。
% 图中所示，为不同相位因子下，不同链路pattern下R值的变化情况。
% 可以看到，b0m1的pattern，在所有相位因子下得到了最低的r，即具有更好的均匀性

% - ------------------     3.3 *Grid 链路组合的吞吐量情况？（暂时不写）----------



% -----------latency and stretch-------------（这段有点难写）
%% outline：
%% 1. +*的对比；
%% vue:链路组合，cdf （链路组合的对比）
%% 结论，b0m1链路组合在f=0时具有最好的能力

% 我们发现， 更均匀的连通性，能有效降低路径连接的绕路情况，以此降低时延。（转折）
% 图中所示为不同链路模式下的 Dijstra路由算法下路径时延和伸张率情况，
% 可以看到：
% 平均时延bm1 < b0 < bm2 < b1
% 在b1,b0链路中，随着相位因子变大，平均时延逐渐增大；在bm1 bm2链路中，随着相位因子增大，逐渐减小。
% 其中，在f=10, bm1的结构中，平均时延达到最低，超过80% 的路径时延不超过为80ms。



% 
% 相应的时延也最低。




% 链路整体最短的是bm1链路，最大的是b1链路
% 在相位因子变大时，bm2链路渐渐降低，b0链路升高，

%在已经有了iISL下，
% +Grid模式下，链路越短，latency越小，stretch 也越小
% hops 在这里没区别。 或者是链路角度分布越均匀stretch越小？
% 想探究CPI路由下的表现？ 


% 测试*Grid模式下的latency和stretch。

% 四种链路，共计有b10,b0m1,bm1m2,b1m1,b0m2,b1m2六种组合。






\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=1.0\linewidth]{fig/polar.png}
    \end{center}
    \caption{Coverage of constellation in different parameters.} 
        \label{fig:polar}
 \end{figure}




 \begin{figure}[htbp]

    \begin{center}
        
    \subfigure[20f00b10m1m2]
    {
    \begin{minipage}{0.44\linewidth}
    \includegraphics[scale=0.2]{fig/20f00b0m1b10bm1m2b1m1b0m2b1m2.png}%以这幅图的0.5倍大小输出
    \end{minipage}
    }\subfigure[20f10b1b0bm1bm2.]
    {
    \begin{minipage}{.44\linewidth}
    \includegraphics[scale=0.2]{fig/20f00b0m1b10bm1m2b1m1b0m2b1m2-str.png}%以这幅图的0.5倍大小输出
    \end{minipage}
    }


\end{center}

   

    \caption{Statistics of eISL between two encountering satellites.} 
       \label{fig:eISL_an}
   \end{figure}


   
 \begin{figure}[htbp]

    \begin{center}
        
    \subfigure[20f00b10m1m2]
    {
    \begin{minipage}{0.44\linewidth}
    \includegraphics[scale=0.2]{fig/b1b0bm1bm2.png}%以这幅图的0.5倍大小输出
    \end{minipage}
    }\subfigure[20f10b1b0bm1bm2.]
    {
    \begin{minipage}{.44\linewidth}
    \includegraphics[scale=0.2]{fig/20f10b1b0bm1bm2.png}%以这幅图的0.5倍大小输出
    \end{minipage}
    }


\end{center}

   

    \caption{Statistics of eISL between two encountering satellites.} 
       \label{fig:eISL_an}
   \end{figure}

==> fwd.tex <==
\author{
	\IEEEauthorblockN{
		Xiangtong Wang\IEEEauthorrefmark{1},
		Wei Li\IEEEauthorrefmark{1}\IEEEauthorrefmark{2},
		Menglong Yang\IEEEauthorrefmark{1}\IEEEauthorrefmark{2}, and
		Songchen Han\IEEEauthorrefmark{1}
		}
		
	% \IEEEauthorblockA{
	% 	\IEEEauthorrefmark{1}School of Aeronautics and Astronautics, Sichuan University, Chengdu, China
	% }

	% \IEEEauthorblockA{
	% 	\IEEEauthorrefmark{2}Robotic Satellite Key Laboratory of Sichuan Province, Chengdu, China
	% }

	% \IEEEauthorblockA{
	% 	Email: \{li.wei, hansongchen\}@scu.edu.cn
	% }
}

\thanks{This paper was produced by the IEEE Publication Technology Group. They are in Piscataway, NJ.}% <-this % stops a space
\thanks{Manuscript received April 19, 2021; revised August 16, 2021.}

% The paper headers
\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2021}%
% {Shell \MakeLowercase{\textit{et al.}}: A Sample Article Using IEEEtran.cls for IEEE Journals}






==> tab/alg.tex <==
\begin{algorithm}
    \label{alg:mplf}
    \caption{Dynamic eISL Configure (DeC) Algorithm }%算法名字
    \LinesNumbered %要求显示行号
    \KwIn{Local coordinates $\mathbf{r}^t(s_0)$ of satellite $s_0$;
    Coordinates $\mathbf{r}^t(s_i)$ of $s_0$;
     Visible satellite set $\mathcal{V}^t_0$;
    Persistent ISL matching matrix $\mathbf{M}^{+},\mathbf{M}^{-}$;
        }%输入参数
  
   
    \KwOut{Encounter matching vector of $s_0$ with its visible satellites $\mathbf{m}^t_{0}$}%输出

    $m_{ij} \leftarrow 0, m_{ij}^t \in M^t$\\
    
       

        \While{  $\mathcal{V}^t_0 \neq \emptyset  $}{

            % \uIf{$\sum\limits_i m^t_{0,i} \textgreater N_e$}{
                % Break;
            % }
            % \ElseIf{Recieve eISL building request from $s_k$}{
                % $m^t_{0,k} \leftarrow 1$;

                % Break;
            % }
           
            Calculate $d(s_0,s_i)$ for all $s_i \in \mathcal{V}_0^t$\\
            $\mathcal{S}_0 \leftarrow \mathop{argsort} \{d(s_0,s_i) \}$;\\
            \For{$s_i \in S_0$ }{
                \uIf{$m^{+}_{0,i} +m^{-}_{0,i} \textgreater 0 $ \textbf{or} $\sum\limits_i m^t_{0,i} \textgreater N_e$}{
                    Continue;
                }
                \ElseIf{$d(s_0,s_i) \leq d_{\delta}$ \textbf{And} $g(s_i,s_j)  \geq g_{\delta}$ \textbf{And} $T(s_0,s_i) \geq T_{\delta}$}{
                    % Send eISL building request to $s_i$;

                    $m^t_{0,i} \leftarrow 1$;
                }    
            }
            update $\mathcal{V}^t_0,~\mathbf{r}^t(s_0),~\mathbf{r}^t(s_i)$;
        }
        
    \end{algorithm}

==> tab/parameters.tex <==
\begin{table}[t!]
	\caption{PARAMETER SETTINGS FOR PERFORMANCE EVALUATION}
	\centering
	\scalebox{0.96}{
		\begin{tabular}{lll}
			\toprule[2pt]
			Parameter          & Symbol    & Setting  \\  \toprule[1pt]
		
			Satellite altitude&$h$&550km\\
			Inclination of the orbital planes &$\delta$  & $53^\circ$ \\
			Satellite Steering Angles&&
		
			% \hline
			Equivalent isotropically radiated power&  ERIP& $31 dBW$ \\
			System bandwidth &$B$&1 GHz\\
			Carrier frequency &$f$&12 GHz\\
			Noise temperature &$T_s$& 324.81K\\

			Scales & $N$ & $10^2, 20^2, 30^2, 40^2$  \\
			Constellation phase factor&$F$& $\{0,\frac{F_m}{8},\frac{F_m}{4},\frac{F_m}{2},F_m\}$\\
			ISL pattern&$\mathcal{B}$&$\{+,* \}$\\
		

			\toprule[2pt]
		\end{tabular}

	}
	\label{tab:param}

\end{table}

==> tab/symbols.tex <==
\begin{table}[]

	\centering
	\scalebox{0.96}{
		\begin{tabular}{lllll}
			\toprule[2pt]
			Density          &$10^2$       &$20^2$ &$30^2$ &$40^2$ \\  \toprule[1pt]
			Throughput& 0.141~Tbps   &1.139~Tbps&3.736~Tbps&8.156~Tbps  \\
			     
			\toprule[2pt]
		\end{tabular}
	}
\end{table}
